Isochrony-Aware Neural Machine Translation for Automatic Dubbing

We introduce the task of isochrony-aware machine translation which aims at generating translations suitable for dubbing. Dubbing of a spoken sentence requires transferring the content as well as the speech-pause structure of the source into the target language to achieve audiovisual coherence. Practically, this implies correctly projecting pauses from the source to the target and ensuring that target speech segments have roughly the same duration of the corresponding source speech segments. In this work, we propose implicit and explicit modeling approaches to integrate isochrony information into neural machine translation. Experiments on English-German/French language pairs with automatic metrics show that the simplest of the considered approaches works best. Results are confirmed by human evaluations of translations and dubbed videos.

==> tables/vc.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \footnotesize
    \tabcolsep=0.10cm
    %\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l c c c c | c  }
        \hline 
        \textbf{Method} & \textbf{BLEU}  & \textbf{ChrF-Phrase}  & \textbf{PPA} & \textbf{PhraseVC} & \textbf{Acceptability} \\
        \hline
        %  MT + PA &  31.2 & 57.9 & 100 & 54.7 & 31.7  \\
        %  MT + [pause] & 32.1 & 58.2 & 98.9 & 55.1 & 32.1    \\
         MT + \textsc{NAR} & 23.5 & 48.6 & 100 & 51.9 & 25.2 \\
         MT + \textsc{LC} & 25.3 & 50.6 & 100 & 54.1 & 27.4 \\
        %  MT + \textsc{Inf. Dis.} & 28.9 & 57.4 & 98.4 & 52.3 & 30.0 \\
        %  MT + \textsc{Inf. Con.} & 31.1 & 58.2 & 98.9 & 55.1 & 32.1 \\
        %  MT + \textsc{Inf. Mask.} & 31.1 & 58.2 & 98.9 & 55.1 & 32.1 \\
        %  MT + \textsc{Post.} & 18.1 & 44. & 99.2 & 38.1 & 16.8 \\
         \hline
    \end{tabular}
    %}
    \caption{Comparing modeling approaches on En-De MustC test set (620 samples). PPA=PauseProjectionAccuracy}%; \textsc{Inf.=} Controlling Verbosity during Inference \textsc{Disc.=} w/ Discrete Steps; \textsc{Inf. Con.=} w/ Continuous Step; \textsc{Inf. Mask.=} w/ Masking}
    % ; \textsc{Post=}  Controlling Verbosity during Post-processing} 
    \label{tab:nar_lc}
\end{table}
